The Gr\"uneisen parameter applied to critical phenomena and experimental investigations of correlated phenomena in molecular conductors

In this Ph.D. Thesis, a systematic review is performed on the derivation and generalization of the Gr\"uneisen parameter followed by its unprecedented applications to several distinct scenarios, such as magnetic model systems, zero-field quantum phase transitions, the maximization of caloric effects close to any critical-end point based on entropy arguments, the here-proposed adiabatic magnetization of a paramagnetic salt, as well as for Cosmology in the frame of the universe expansion. Since this Ph.D. Thesis is a symbiosis between theoretical and experimental results, an experimental investigation of correlated phenomena was carried out for molecular conductors of the (TMTTF)$_2$X family, where TMTTF is the base molecule tetramethyltetrathiafulvalene and X a monovalent counter-anion such as PF$_6$, SbF$_6$, or AsF$_6$. Such strongly correlated electron systems are considered suitable ones for the exploration of Mott insulating phase, charge-ordering, spin-Peierls, and superconductivity. In particular, the investigation of a possible multiferroic character in these salts was performed via quasi-static (low-frequency) dielectric constant $\varepsilon'$ measurements as a function of temperature where a maximum in $\varepsilon'$ as a function of temperature was observed at the corresponding charge-ordering temperature for both hydrogenated and 97.5% deuterated (TMTTF)$_2$SbF$_6$ salts. Furthermore, Raman measurements were performed on the 97.5% deuterated (TMTTF)$_2$PF$_6$, showing a possible magneto-optical effect on the $\nu_4(a_g)$ vibrational mode of the TMTTF molecule. Yet, fluorescence measurements demonstrated that the fully-hydrogenated (TMTTF)$_2$AsF$_6$ presents an expressive fluorescence background, which is roughly five orders of magnitude lower than that for the 97.5% deuterated variant of (TMTTF)$_2$PF$_6$.

==> text/abbreviations.tex <==
% First parameter can be changed eg to "Glossary" or something.
% Second parameter is the max length of bold terms.
\begin{mclistof}{List of Abbreviations}{3.2cm}

\item[1-D, 2-D] One- or two-dimensional, referring in this thesis to spatial dimensions in an image.

\item[Otter] One of the finest of water mammals.

\item[Hedgehog] Quite a nice prickly friend.

\end{mclistof} 


==> text/jointreports.tex <==
\chapter{Participation in joint reports}

During 








==> text/resumo.tex <==
Fenômenos críticos são de grande interesse para a comunidade científica e podem ser estendidos para várias áreas de pesquisa, como transições de fase clássicas e quânticas, efeitos calóricos e até mesmo na Biologia no contexto da funcionalidade cerebral, por exemplo. É discutido amplamente na literatura que a grandeza física crucial para se acessar experimentalmente tanto pontos críticos a temperatura finita quanto pontos críticos quânticos é a chamada razão Gr\"uneisen. Nesta tese de doutorado, uma revisão sistemática é realizada sobre a derivação e generalização do parâmetro de Gr\"uneisen seguido pelas suas aplicações inéditas para diversos cenários físicos distintos, tais como sistemas modelo para o magnetismo, transições de fase quântica a campo magnético zero, a maximização de efeitos calóricos próximos de qualquer ponto crítico baseado em argumentos de entropia, para a magnetização adiabática de um sal paramagneto proposta nesta tese, bem como para a Cosmologia no contexto da expansão do universo. Uma vez que esta tese de doutorado é uma simbiose entre resultados experimentais e teóricos, uma investigação experimental de efeitos correlacionados em condutores moleculares também foi realizada para os condutores moleculares da família (TMTTF)$_2$X, onde TMTTF é a molécula base tetrametiltetratiafulvaleno e X um contra-ânion monovalente, tais como PF$_6$, SbF$_6$ ou AsF$_6$. Tais sistemas eletrônicos fortemente correlacionados são considerados apropriados para a exploração de isolantes de Mott, fase de carga ordenada, spin-Peierls e até mesmo supercondutividade. Em particular, uma investigação do possível caráter multiferroico destes sais foi realizada utilizando medidas de constante dielétrica quase estática (baixa frequência) $\varepsilon'$ em função da temperatura onde um máximo de $\varepsilon'$ foi observado na temperatura de ordenamento de carga correspondente para a variante totalmente hidrogenada e 97,5\% deuterada do sal (TMTTF)$_2$SbF$_6$. Além disso, experimentos Raman foram realizados na variante 97,5\% deuterada do sistema (TMTTF)$_2$PF$_6$, onde um possível efeito magneto-óptico no modo vibracional $\nu_4(a_g)$ da molécula TMTTF foi observado. Ainda, experimentos adicionais mostraram que o sistema totalmente hidrogenado (TMTTF)$_2$AsF$_6$ apresenta uma expressiva fluorescência, a qual é cerca de cinco ordens de magnitude maior do que a da variante 97,5\% deuterada do sistema (TMTTF)$_2$PF$_6$.
\newline\newline
Palavras-chave: fenômenos críticos; parâmetro de Gr\"uneisen; sistemas eletrônicos fortemente correlacionados. 
